Viewing the process of generating counterfactuals as a source of knowledge: a new approach for explaining classifiers

There are now many explainable AI methods for understanding the decisions of a machine learning model. Among these are those based on counterfactual reasoning, which involve simulating features changes and observing the impact on the prediction. This article proposes to view this simulation process as a source of creating a certain amount of knowledge that can be stored to be used, later, in different ways. This process is illustrated in the additive model and, more specifically, in the case of the naive Bayes classifier, whose interesting properties for this purpose are shown.

==> old_files/concepts.tex <==
\section{Concepts}
\label{sec-concepts}

%On présente ci-dessous certains concepts clefs qui seront utilisés dans la suite de cet article.

\subsection{Countrefactual and semi-factual example}

In machine learning, a counterfactual explanation aims to explain why a particular result was obtained by suggesting hypothetical changes in the input features $X$ that might have led to a different prediction \cite{LemaireIGI2010correlation,wachter2018counterfactual}.
%\cite{wachter2018counterfactual}. 
In other words, it identifies the factors that could have influenced a particular outcome. Counterfactual reasoning can be defined as follows:

\begin{definition}
Let $f$ be $\mathcal{X} \mapsto \mathcal{Y}$ a machine learning model such that, for a given individual $X$, $f(X)=\hat{y}_i$. In this case, a counterfactual example is a new example $X'$ such that $f(X') \neq \hat{y}_i$ and $X \neq X'$. If $X$ had different values for some of its explanatory variables ($X_1', X_2', ...$) while all the other variables remained identical, the class $\hat{y}_j \neq \hat{y}_i$ would have been returned.
\end{definition}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.3\textwidth]{schema_contrefactuel_semi.PNG}\
    \caption{Illustration of a counterfactual and a semi-factual. The red dots represent initial examples ($X$). The orange dot represents a semi-factual, the purple dot represents a counterfactual and the white line represents the decision boundary between the red and green classes.}
    \label{fig1}
\end{figure}

Above, $\hat{y}_i$ is known and factual, while $\hat{y}_j$ is the unexpected result that did not happen, counterfactual. Note, however, that a change from $X$ to $X'$ does not necessarily lead to a change in the class prediction: this is known as a semi-factual example \cite{fernandez2022explanation}. The knowledge of counterfactual or semi-factual examples makes it possible to explain how to change, to modify, the decisions of the model: ``Your bank loan was not accepted BUT IF you had more seniority in our company, the decision would have been the opposite (or closer to acceptance)". These two concepts are illustrated in Figure 1. The understanding produced by a ``counterfactual" method of explanation is local, because it applies to a particular individual, and ``instance-based", because it is produced in the form of a new example.



\subsection{Informativeness and actionability of variables}
\label{info}

In decision making, and particularly in the context of counterfactual reasoning, the identification of informative and actionable variables is essential. An informative variable is defined as a variable that has a significant impact on the value of the output of the predictive model.
%
However, it is not enough to know which variables are informative. It is also important to identify the actionable variables, which we define as a variable on which it is possible to act.
%
The most valuable type of variable is the actionable informative variable, i.e. one that not only has a significant impact on the output variable, but can also be acted upon to improve or influence the result. 
%Une telle variable est aussi appelée `variable à effet de levier' \cite{LemaireIGI2010correlation}. 

%Note: puisque, dans cet article, il s'agit de générer des exemples contrefactuels, il est intéressant de considérer ci-dessus la notion d'influence au niveau local (exemple par exemple) et non au niveau global (pour le modèle en général). 

\subsection{The concept of trajectories}
\label{subsec-traj}

The scientific literature offers numerous methods for generating counterfactual examples, either model dependent (depending on the type of classifier) or agnostic to the predictive model %\cite{stepin2021survey,wachter2018counterfactual,nice,Guyomard}.
\cite{stepin2021survey,nice}. In this article we are interested in methods that induce the notion of trajectory. If we take Figure \ref{fig1}, we are interested in methods which allow us to approach the decision frontier step by step (until $X$ cross it) by successive modifications of the initial example. %footnote{We can imagine, for example, that additive predictive models are good candidates}.
In this case, the succession of $X'$ resulting from these successive operations is called a `trajectory' (see Figure 2).


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.3\textwidth]{schema_contrefactuel_semi_trajectoire.PNG}\
    \caption{Illustration of two counterfactuals: one achieved in 1 step, the second in 3 steps}
    \label{fig2}
\end{figure}

Over the course of this article, we will be particularly interested in predictive methods and/or models that allow for a notion of additivity in this trajectory. That is, the univariate modifications of $X$ add up and make it possible to approach the decision frontier by variable-by-variable modification, step by step, as shown in Figure 2. We will show later that this is the case for the Naive Bayes classifier.

==> old_files/database.tex <==
\section{Creation and use of a knowledge base}
\label{sec-knowledge}

\subsection{Creation a knowledge base}

In the foregoing we have shown how to increase the probability of belonging to a class of interest and quantify this increase using the equation \ref{eq-delta}. We have also shown that this quantity is additive as we change the values of the explanatory variables one by one. We now propose to store these $\Delta$ values in a table in the form shown in Table \ref{Table-delta-1}.

It should be remembered that it is assumed that the numerical variables have been discretised beforehand and that a grouping of modalities has been carried out for the categorical variables. Each variable is therefore represented by a limited number of values (corresponding to the values of $P(X|C)$). Table \ref{Table-delta-1} gives, for illustrative purposes, the values stored in the case where the predictive model uses two explanatory variables $X_1$ and $X_2$ respectively discretised (or grouped) into 3 and 2 intervals (groups) of values ($I$). For each individual, $l$, each row of the table, we store the values of the equation \ref{eq-delta} where $\Delta(X^{l}_{i,*\rightarrow m}, X^l)$ is the value of $\Delta$ when the value of variable $i$ is changed from its initial value $`*'$ to the value of interval (group) $m$ (simplified as $\Delta(X^{l}_{i,*\rightarrow m})$ in the table).
\vspace{-3mm}

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{|c|}{$X_1$}    &  \multicolumn{3}{|c|}{$X_2$} \\\hline
&  $I_1$  & $I_2$  & $I_1$ & $I_2$ & $I_3$ \\\hline
${X^1}$ & $\Delta({X^{1}_{1,*\rightarrow 1}})$ & $\Delta({X^{1}_{1,*\rightarrow 2}})$ & $\Delta({X^{1}_{2,*\rightarrow 1}})$ & $\Delta({X^{1}_{2,*\rightarrow 2}})$ & $\Delta({X^{1}_{2,*\rightarrow 3}}$ \\\hline
${X^2}$ & $\Delta({X^{2}_{2,*\rightarrow 1}})$ & $\Delta({X^{2}_{2,*\rightarrow 2}})$ & $\Delta({X^{2}_{2,*\rightarrow 1}})$ & $\Delta({X^{2}_{2,*\rightarrow 2}})$ & $\Delta({X^{2}_{2,*\rightarrow 3}})$ \\ \hline
\end{tabular}
\end{center}
\caption{Illustration of the knowledge base created in the form of $\Delta$, here in the case of two variables and two examples.}
\label{Table-delta-1}
\end{table}
\vspace{-8mm}

We detail in the following sections how to exploit the knowledge stored in this way. In this article, only the naive Bayes classifier is considered, but any other classifier and/or counterfactual creation method that produces a similar data table could be used.

\vspace{-3mm}
\subsection{Generation of counterfactuals with certain properties}

\subsubsection{Minimising the number of changes - }
We can set ourselves the criterion of finding the counterfactual with the property of involving the smallest number of modified variables.
To do this, we will exploit the knowledge base. 
For a given individual, $X$, all we have to do is read the value of the largest $\Delta$ and then, as we have the additivity property, read the second value of the largest $\Delta$ for a second variable and so on.
At each stage we check whether ($\hat{f}(\mathbf{X'}) > 0.5$). If this is the case, the counterfactual has been found footnote{We could, on the other hand, maximise the number of changes, but this is often of little interest in practice}.
\vspace{-3mm}

\subsubsection{Taking account of business constraints or criteria - }
In other cases, the aim may be to find the closest counterfactual, but under `business constraints' defined by the user. For example, the search for counterfactuals could be restricted to making changes only in adjacent intervals (e.g. intervals of close values). Given the table \ref{Table-delta-1}, we would be allowed to move people from interval 1 to 2 for the second variable, but not from 1 to 3. The user can also constrain the search by requiring that one of the variables must always be changed to a certain value, and so on. This type of constraint can easily be considered and incorporated into a counterfactual search algorithm using the proposed knowledge table.

The literature on counterfactuals sets out some interesting properties on the subject, such as (i) the notion of minimality: having a counterfactual that differs as little as possible from the original example; (ii) realism: the generated counterfactual must not contain changes that do not make sense from the point of view of the data (e.g. a decrease in the ``age" of an individual), also known as plausibility \cite{pmlr-v180-nemirovsky22a}; (iii) generating counterfactuals that are similar to real examples or in dense regions of the class of interest, in order to have robust counterfactuals \cite{guyomard2023generating}; in this case, in the case of the naive Bayes classifier, we can use a Bayesian distance as proposed in \cite{pkmean}; ...

All these properties are easily achieved with the Table \ref{Table-delta-1}, since the user can choose the list and the order of the variables he wish to intervene on, as well as a distance of his choice between $X$ and $X'$.
\vspace{-3mm}

\subsection{Additional usable knowledge}
\subsubsection{Preventive and reactive actions - }

So far, we have mainly talked about creating counterfactuals to explain the model's decisions (as mentioned in the introduction to this article), but potentially also to be able to take reactive actions. For example, if a bank customer is predicted to "leave" (churner), the counterfactual example indicates one or more actions to be taken in order to try to keep him as a customer: these are known as {\bf ``reactive" actions}.

Conversely, the study of counterfactual trajectories a posteriori is of great interest, as it also allows us to identify when a trajectory is approaching the frontier. In such situations, reactive measures can be taken to reverse the trend and avoid undesirable outcomes. This approach is particularly relevant when it comes to predicting churn, for example, as it enables us to identify customers who are ``starting'' to churn. By being proactive, it is possible to put in place targeted strategies to retain these customers and bring them back to a quality service. 

Finally, our knowledge base can also be used to carry out {\bf ``preventive" actions}. Going back to Figure 1, we can try to create a semi-factual which moves away from the decision frontier: "The customer is not predicted as leaving but is nevertheless close to the decision frontier". In this case, all we need to do is look at the negative values of $\Delta$ and take steps away from it according to the user's wishes. For example, all the people who are one step away from crossing the decision frontier, who are easily identifiable in this case, could be concerned.\vspace{-4mm}


\subsubsection{Profile creation - }

The last way of using the knowledge base that we will describe here\footnote{The reader can imagine others: descriptive statistics of the table, number of individuals at 1, 2, 3 ... steps from the decision frontier, visualisation of the trajectories, ... .}, is to carry out an exploratory analysis using a clustering technique.
%
Using the knowledge base, it is possible to group individuals according to the impact of each possible change, i.e. the impact resulting from each of these changes. Analysis of the clusters created can be a source of learning. This is illustrated in the next section. 


%\subsubsection{Statistiques descriptives}

==> old_files/introduction_victor.tex <==
%-------------------------------------------------------
\section{Introduction}
\label{sec-introduction}


Machine learning, a branch of artificial intelligence, has witnessed numerous successes in recent years. However, these achievements have come at the cost of increasingly complex models, where the decision process becomes opaque. Thus, it became impossible for the users to understand why the model outputs a given prediction. 
This has given rise to eXplainable AI (XAI), a field aimed at making machine learning decisions intelligible and user-friendly.


% Le potitionnement !! 




In this spirit, we propose a framework for enhancing the explanatory capabilities of interpretable models by offering various types of explanations, including counterfactual explanations, trajectories, and clustering analysis.
Our framework relies on the construction of a knowledge base that stores the impact of different feature changes to the predictions. 

We illustrate the advantages of our framework through a churn prediction task, showcasing its particular value in identifying practical actions to reduce churn and facilitating discussions with the business team to gain deeper insights into diverse customer profiles.

In what follows, we will focus specifically on the naive Bayes classifier, however this choice has no limitation as our method can be extended to additive classifiers. 









==> old_files/nb.tex <==
\section{Optimised search for counterfactuals in the case of the naive Bayes classifier}
\label{sec-nb}

%Petit préambule à jouter pour décrire les parties de la section ?


\subsection{Reminders on the naive Bayes classifier}

The naive Bayes classifier (NB) is a widely used tool in supervised classification problems. It has the advantage of being efficient for many real data sets \cite{Hand2001}. However, the naive assumption of conditional independence of the variables  can, in some cases, degrade the classifier's performance. This is why variable selection methods have been developed \cite{Langley1994}. They mainly consist of variable addition and deletion heuristics to select the best subset of variables maximizing a classifier performance criterion, using a wrapper-type approach \cite{Guyon2003}. It has been shown %in \cite{BoulleJMLR07} 
that averaging a large number of selective naive Bayes classifiers, performed with different subsets of variables, amounts to considering only one model with a weighting on the variables. Bayes' formula under the assumption of independence of the input variables conditionally to the class variable becomes:

\begin{equation}
P(C_{k}|X)=\frac{P(C_{k})\prod_{i}P(X_{i}|C_{k})^{W_i}}{\sum_{j=1}^{K}(P(C_{j})\prod_{i}P(X_{i}|C_{j})^{W_i})}
\label{snb}
\end{equation}

where $W_i \in [0, 1]$ is the weight of variable $i$.
The predicted class is the one that maximizes the conditional probability $P(C_{k}|X)$. The probabilities $P(X_i|C_i)$ can be estimated by interval using discretization for numerical variables. Gaussian naive Bayes could be also considered. For categorical variables, this estimation can be done directly if the variable takes few different modalities, or after grouping (of values) in the opposite case. 



\subsection{Criteria to be optimised in the search for counterfactuals}

Let, $X$ as an example, and two classes $C_1$ and $C_2$. The search for a counterfactual consists in optimising and increasing the probability of belonging to the target class $C_1$ when $X$ is initially predicted by the model to belong to $C_2$ (and vice versa). To do this, we can develop a gluttonous algorithm, which is expensive in terms of computation time and does not necessarily have the additivity properties described above in Section \ref{subsec-traj}. We propose below to pose the problem differently, rewriting the equation \ref{snb} and looking at how to increase the probability of belonging to a particular class of interest. To achieve this goal, and to maximise $P(C_j|X')$ with respect to the initial value of $P(C_j|X)$, we will exploit the following proposition:

\begin{proposition}
If we take $X$ and $X'$ as two elements of the input space $\mathcal{X}$, we show that for a two-class classification problem, searching for counterfactuals of $X$ amounts to examining the evolution of the value of $\Delta$ when we change some of the values of $X$ to $X'$, such that:

\begin{equation}
\begin{split}
\Delta(X, X') &= \left( \sum_{i=1}^d W_i(\log{P(X_i|C_{1})}  - \log{P(X_i |C_{2})}) \right)\\ & - \left(  \sum_{i=1}^d W_i(\log{P(X'_i|C_{1})} - \log{P(X'_i |C_{2})}) \right)
\end{split}
\label{eq-delta}
\end{equation}
\end{proposition}

{\it Proof:} If we start again from the equation \ref{snb}
$$P(C_j|{X}) = \frac{P(C_j)\prod_{i=1}^dP(X_i|C_j)^{W_j}}{\sum_{z}[P(C_z)\prod_{i=1}^dP(X_i|C_z)^{W_j}]}$$

by posing: 

\begin{equation*}
\small
L_j({X}) = \log \left( P(C_j)\prod_{i=1}^dP(X_i|C_j)^{W_i} \right) = \log{P(C_j)} + \sum_{i=1}^d W_i\log{P(X_i|C_j)}, 
\end{equation*}


then we have:

$$P(C_j|{X}) = \frac{e^{L_j({X})}}{\sum_{z}e^{L_z({X})}} = \frac{1}{\sum_{z}e^{L_z({X}) - L_j({X})}} = \frac{1}{1 + \sum_{z \neq j}e^{L_z({X}) - L_j({X})}}$$

and so in the case of two classes:

\begin{equation}
P(C_j|{X}) = \frac{1}{1 + e^{L_{j'}({X}) - L_j({X})}}
\label{eq-norm}
\end{equation}

We can see that to get closer to the class $C_j$, all we have to do is reduce the quantity $L_{j'}({X}) - L_j({X})$, and thus reduce:


$$\log{P(C_{j'})} + \sum_{i=1}^d W_i\log{P(X_i|C_{j'})} - \log{P(C_j)} - \sum_{i=1}^d W_i\log{P(X_i|C_j)}$$

Since $P(C_{j})$ and $P(C_{j'})$ are constant, this is equivalent to decreasing: $$\sum_{i=1}^d W_i\log{P(X_i|C_{j'})} - \sum_{i=1}^d W_i\log{P(X_i|C_{j})}$$

and therefore to take an interest in the distance:

\begin{equation*}
\begin{split}
\Delta({X}, {X'}) &= \sum_{i=1}^d W_i(\log{P(X_i  |C_{j'})} - \log{P(X_i |C_{j})}) \\
&- \sum_{i=1}^d W_i(\log{P(X'_i  |C_{j'})} - \log{P(X'_i  |C_{j})})
\end{split}
\end{equation*}


%\textcolor{red}{intéret de $A_ik$ ci-dessus ?}

If $\Delta$ is positive then we are getting closer to the decision frontier (or even crossing it) if $\Delta$ is negative then we are moving away from the decision frontier and therefore away from the desired objective. The counterfactual search algorithm becomes straightforward. Simply calculate, for a given example $X$, the value of $\Delta$ for each explanatory variable and for each value of this explanatory variable. Then, given these values, iterate the successive changes in order to obtain a counterfactual example. These variable-by-variable changes have the property of being additive.  

Indeed, if we consider four examples $X^0$, $X^{'1}$, $X^{'2}$ and $X^{'3} \in \mathcal{X}$, which are respectively (i) an initial example $X^0$, then the same example for which we have modified only one explanatory variable $l$ for $X^{'1}$, $m$ for $X^{'2}$, and finally an example that cumulates the two univariate modifications $l$ and $m$ for $X^{'3}$, such that :


$$\exists! \ l \ \text{such as} \ X^{'1}_l \neq X^{0}_l$$

$$\exists! \ m \ \text{such as} \ X^{'2}_m \neq X^{0}_m \ \text{and} \ m \neq l$$

and $$ X^{'3}_k = \begin{cases}
    X^{'1}_l, & \text{if } k=l \\
    X^{'2}_m, & \text{if } k=m \\
    X^{0}_k, & \text{otherwise}
\end{cases}
$$

then it is obvious, from the additivity over all the variables in the equation \ref{eq-delta}, that we have : $\Delta({X_0},{X'_3}) = \Delta({X_0},{X'_1}) + \Delta({X_0},{X'_2})$. Modifying one variable and then the other is equivalent to modifying them simultaneously in the calculation of $\Delta$. It should also be noted that this additivity is demonstrated from the equation \ref{eq-norm}, so we can be sure of increasing the value {\bf normalised} of the probability of the class of interest, $P(C|X)$, which is a plus.

Note: The list of $\Delta$ values can potentially be very large if the number of distinct values of the explanatory variables is large. Nevertheless, it is common for some naive Bayes classifiers (except the Gaussian version) \cite{Yang2003,Yang2009} to discretise the numerical variables and group the modalities of the categorical variables, in a supervised manner, in order to obtain an estimate of the conditional densities ($P(X_i|C)$) which are then used in the calculation of $P(C|X)$.
%This is what has been done in this article using the \cite{BoulleML06} and \cite{BoulleJMLR05} methods for numerical and categorical variables respectively. 
These supervised discretisation and grouping operations often produce a limited number of intervals or groups of modalities. This makes it possible to obtain a reasonable number of values to test.

